The observed impact of galaxy halo gas on fast radio bursts

Galaxies and groups of galaxies exist in dark-matter halos filled with diffuse gas. The diffuse gas represents up to 80\% of the mass in baryonic matter within the halos(1,2), but is difficult to detect because of its low density (particle number densities of $\lesssim10^{-4}$\,cm$^{-3}$) and high temperature (mostly greater than $10^{6}$\,K). Here we analyze the impact of diffuse gas associated with nearby galaxies using the dispersion measures (DMs) of extragalactic fast radio bursts (FRBs). FRB DMs provide direct measurements of the total ionized-gas contents along their sightlines. Out of a sample of 474 distant FRBs from the CHIME/FRB Catalog 1(3), we identify a subset of events that likely intersect the dark-matter halos of galaxies in the local Universe ($<40$\,Mpc). The mean DM of the galaxy-intersecting FRBs is larger than the non-intersecting DMs with probability $>0.99$ and the excess DM is $>90$\,pc\,cm$^{-3}$ with $>95\%$ confidence. The excess is larger than expected for the diffuse gas surrounding isolated galaxies, but may be explained by additional contributions from gas surrounding galaxy groups, including from the Local Group. This result demonstrates the predicted ability of FRBs to be used as sensitive, model-independent measures of the diffuse-gas contents of dark-matter halos(4-7).

==> incl-authors.tex <==
%% -- Your edits may get overwritten by the formatting script -- check with JVL -- 

%% ----------------- Authors ---------------
%% -- One-liner for submission form, etc. --
%% In\'es Pastor-Marazuela, Liam Connor, Joeri van Leeuwen, Yogesh Maan, Sander ter Veen, Anna Bilous, Leon Oostrum, Emily Petroff, Samayra Straal, Dany Vohl, Jisk Attema, Oliver M. Boersma, Eric Kooistra, Daniel van der Schuur, Alessio Sclocco, Roy Smits,Elizabeth A. K. Adams, Bj\"orn Adebahr, Willem J.G. de Blok, Arthur H. W. M. Coolen, Sieds Damstra, Helga D\'enes , Kelley M. Hess, Thijs van der Hulst, Boudewijn Hut, V. Marianna Ivashina, Alexander Kutkin, G. Marcel Loose, Danielle M. Lucero, \'Agnes Mika, Vanessa A. Moss, Henk Mulder, Menno J. Norden, Tom Oosterloo, Emanuela Orr\'u, Mark Ruiter, Stefan J. Wijnholds 
%% -- All author acronyms for contributions etc --
%% IPM, LC, JVL, YM, STV, AB, LO, EP, SS, DV, ABAO, JA, OB, EK, DVDS, AS, RS, AB&P, EAKA, BA, WJDB, AHWMC, SD, HD, KMH,
%% TVDH, BH, VMI, AK, GML, DML, AM, VAM, HM, MJN, TO, EO, MR, SJW 
%% -- Latex formatted ------------------- --
\author{%
Liam~Connor$^1$,
Vikram~Ravi$^{1,2}$
} 

